conv_einsum: A Framework for Representation and Fast Evaluation of Multilinear Operations in Convolutional Tensorial Neural Networks

Modern ConvNets continue to achieve state-of-the-art results over a vast array of vision and image classification tasks, but at the cost of increasing parameters. One strategy for compactifying a network without sacrificing much expressive power is to reshape it into a tensorial neural network (TNN), which is a higher-order tensorization of its layers, followed by a factorization, such as a CP-decomposition, which strips a weight down to its critical basis components. Passes through TNNs can be represented as sequences of multilinear operations (MLOs), where the evaluation path can greatly affect the number of floating point operations (FLOPs) incurred. While functions such as the popular einsum can evaluate simple MLOs such as contractions, existing implementations cannot process multi-way convolutions, resulting in scant assessments of how optimal evaluation paths through tensorized convolutional layers can improve training speed. In this paper, we develop a unifying framework for representing tensorial convolution layers as einsum-like strings and a meta-algorithm conv_einsum which is able to evaluate these strings in a FLOPs-minimizing manner. Comprehensive experiments, using our open-source implementation, over a wide range of models, tensor decompositions, and diverse tasks, demonstrate that conv_einsum significantly increases both computational and memory-efficiency of convolutional TNNs.

==> tex/fig_reshaping.tex <==
\begin{wrapfigure}{r}{70mm}
    \vspace{-0.5em}
    \centering
    \includegraphics[width=0.3\textwidth]{\fighome/modularity.pdf}
    \vspace{-0.5em}
    \caption{\textbf{Tensor reshaping.} 
    Reshaping can help reduce the number of parameters while preserving critical structural properties. A vector of length 15 displays periodicity in its entries (represented here by repeating colors) except for a few entries. Reshaping it into a $3\times 5$ matrix and then taking a factorized tensor approximation (rank-1 SVD) \textbf{a)} reduces the number of parameters to store and \textbf{b)} culls out artifacts (non-periodic elements) while representing periodicity sans redundancy.
    }
\label{fig:periodicity}
\vspace{-1em}
\end{wrapfigure}

==> tex/figure_conv_layer.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{\fighome/convdrawio.pdf}
    \vspace{-1.5em}
    \caption{\textbf{Depiction of a standard convolutional layer.} 
    Here $\mytensor{U} \in \R^{N\times X \times Y}$ is an $N$-stacked batch of $X\times Y$ images (Vincent van Gogh's \textit{Portrait of Joseph Roulin}). This batch is fed through a $4^\th$-order convolutional tensor $\mytensor{K}\in\R^{N \times C \times H \times W}$, where $H$ and $W$ are the kernel height and width, respectively, and $C$ is the number of output channels. (The kernel has been decomposed along its output channel mode by its matricized slices. Furthermore, we are not depicting the $N$-dimensional batch mode of each slice.) After a max-padded blurring convolution between the mode pairs $(X,H)$ and $(Y,W)$ and contraction over the $N$-dimensional batch mode, the output is a third order tensor $\mytensor{Y} \in\R^{X \times Y \times C}$.}
    \label{fig:conv-layer}
\end{figure}

==> tex/performance_rcp.tex <==
\begin{figure}[!htbp]
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
  \input{\texhome/video_rcp_performance}
    }
\subcaption{Image Classification}\label{fig:image-performance-rcp}
\end{minipage}%
\hfill
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
    \input{\texhome/video_rcp_performance}
    }
\subcaption{Speech recognition}\label{fig:speech-performance-rcp}
\end{minipage}%
\hfill
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
    \input{\texhome/video_rcp_performance}
    }
\subcaption{Video Classification}\label{fig:video-performance-rcp}
\end{minipage}
\caption{Performance}\label{fig:performance-rcp}
\end{figure}



==> tex/runtime_cifar-rcp.tex <==
\begin{figure}[!htbp]
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
   \input{\texhome/image_cls_rcp_train}
    }
\subcaption{RCP Train}\label{fig:imagecls-rcp-vs-pytorch-train}
\end{minipage}%
\hfill
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
    \input{\texhome/image_cls_rcp_test}
    }
\subcaption{RCP Test}\label{fig:imagecls-rcp-vs-pytorch-test}
\end{minipage}
\caption{\textbf{Runtime comparison between \conveinsum and \pytorch for an image classification task.} An RCP-TNN ($R=3$) is trained on the CIFAR-10 dataset. Runtimes are averaged over 3 random runs, and error bars are denoted by the shaded areas.}\label{fig:imagecls-rcp-vs-pytorch}
\vspace{-1em}
\end{figure}

==> tex/runtime_cifar_cp.tex <==
\begin{figure}[!htbp]
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
   \input{\texhome/image_cls_cp_train_lib_vs_pytorch_tensor}
    }
\subcaption{CP Train}\label{fig:imagecls-cp-vs-pytorch-train}
\end{minipage}%
\hfill
\begin{minipage}[b]{.5\linewidth}
\centering
\resizebox{\textwidth}{!}{
    \input{\texhome/image_cls_cp_test_lib_vs_pytorch_tensor}
    }
\subcaption{CP Test}\label{fig:imagecls-cp-vs-pytorch-test}
\end{minipage}
\caption{Run-time comparison between \texttt{conv\_einsum} and \texttt{Pytorch} implementation of CP-TNN for image classification machine learning task implemented on CIFAR-10 dataset. We denote error bars using shaded areas and they are generated using 10 random runs. }\label{fig:imagecls-cp-vs-pytorch}
\end{figure}

==> tex/tab_video_max_batch_size.tex <==
\begin{table}[!htbp]
\vspace{-1em}
\caption{\textbf{Maximum batch size for a video classification task for spatial (S) and temporal (T) streams of two-stream network.} The maximal batch size allowed for data under varying compression rates and using different libraries. "ckpt" = checkpointing. %using \texttt{conv\_einsum} and \pytorch with/without checkpointing.
}
 \label{tab:video-max-batch-size}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{2}{c}{\conveinsum} & \multicolumn{2}{c}{\shortstack{\pytorch w/ ckpt}} & \multicolumn{2}{c}{\shortstack{\pytorch w/o ckpt}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    \thead{CR} & \thead{S} & \thead{T} & \thead{S} & \thead{T} & \thead{S} & \thead{T}\\
    \midrule
    1\% & 20 & 30 & 2 & 4 & 1 & 2\\
    2\% & 20 & 30 & 2 & 4 & 0 & 0\\
    5\% & 20 & 30 & 2 & 4 & 0 & 0\\
    10\% & 18 & 30 & 1 & 2 & 0 & 0\\
    20\% & 16 & 27 & 0 & 0 & 0 & 0\\
    50\% & 12 & 22 & 0 & 0 & 0 & 0\\
    100\% & 4 & 14 & 0 & 0 & 0 & 0\\
    \bottomrule
 \end{tabular}}
 \vspace{-1em}
\end{table}

==> tex/table_operations_comparison.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:operations-comparison}
\end{table}

==> tex/table_primitive_operations.tex <==
\begin{table}[!htbp]
\centering
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c c c}
\toprule
Operator & Notation & Definition \\
\midrule
	% 1) tensor contraction
	\begin{tabular}{l} mode-($I_k, J_l$) \\ Tensor Contraction \end{tabular} & 
	$\tensorSup{T}{1} = \tensor{X} \times^{I_k}_{J_l} \tensor{Y}$ &
	\begin{tabular}{l} $\tensorInd{T}{i_0, \cdots, i_{k-1}, i_{k+1}, \cdots, i_{m-1}, j_0, \cdots, j_{l-1}, j_{l+1}, \cdots, j_{n-1}}{1}$ \\
	$ = \big< \tensorSub{X}{i_0, \cdots, i_{k-1},{ :}, i_{k+1}, \cdots, i_{m-1}},  \tensorSub{Y}{j_0, \cdots, j_{l-1}, {:}, j_{l+1}, \cdots, j_{n-1}}\big>$ \\ 
	Inner product of mode-$k$ fiber of $\tensor{X}$ and mode-$l$ fiber of $\tensor{Y}$ \end{tabular} \\
\midrule
	% 2) tensor convolution
	\begin{tabular}{l} mode-$(I_k, J_l)$ \\Tensor Convolution \end{tabular} & 
	$\tensorSup{T}{2} = \tensor{X} \ast^{I_k}_{J_l} \tensor{Y}$ &
	\begin{tabular}{l}$\tensorInd{T}{i_0, \cdots, i_{k-1}, {:}, i_{k+1}, \cdots, i_{m-1}, j_0, \cdots, j_{l-1}, j_{l+1}, \cdots, j_{n-1}}{2} $ \\
	$= \tensorSub{X}{i_0, \cdots, i_{k-1}, {:}, i_{k+1}, \cdots, i_{m-1}} \ast \tensorSub{Y}{j_0, \cdots, j_{l-1},{ :}, j_{l+1}, \cdots, j_{n-1}}$ \\ 
	Convolution of mode-$k$ fiber of $\tensor{X}$ and mode-$l$ fiber of $\tensor{Y}$ \end{tabular} \\
\midrule
	% 3) tensor outer product
	\begin{tabular}{l} mode-($I_k, J_l)$ \\ Tensor Batch Product \end{tabular} &
	$\tensorSup{T}{3} = \tensor{X} \otimes^{I_k}_{J_l} \tensor{Y}$ & 
	\begin{tabular}{l} $\tensorInd{T}{i_0, \cdots, i_{k-1}, {r}, i_{k+1}, \cdots, i_{m-1}, j_0, \cdots,  j_{n-1}}{3} $ \\
	$=\tensorSub{X}{i_0, \cdots, i_{k-1}, {r}, i_{k+1}, \cdots, i_{m-1}} ~ \tensorSub{Y}{j_0, \cdots, j_{l-1},{ r}, j_{l+1}, \cdots, j_{n-1}}$ \\ 
	Hadamard product of mode-$k$ fiber of $\tensor{X}$ and mode-$l$ fiber of $\tensor{Y}$ \end{tabular} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Primitive tensor operations}. 
$\tensor{X} \in \R^{I_0 \times \cdots \times I_{m-1}}$, 
$\tensor{Y} \in \R^{J_0 \times \cdots \times J_{n-1}}$ are input tensors.
$\tensorSup{T}{1}$, $\tensorSup{T}{2}$, $\tensorSup{T}{3}$ are the outputs of 
Mode-$(I_k, J_l)$ tensor contraction, tensor convolution, and batch outer product.
Note that both mode-$(I_k, J_l)$ tensor contraction and mode-($I_k, J_l$) tensor batch product 
are legal only if $I_k = J_l$. Consequently, $\tensorSup{T}{1}$ is an $(m+n-2)$-order tensor
and $\tensorSup{T}{2}$, $\tensorSup{T}{3}$ are $(m+n-1)$-order tensors.}
\label{tab:primitive-operations}
\end{table}
